Prefixing Attention Sinks can Mitigate Activation Outliers for Large Language Model Quantization

Despite recent advances in LLM quantization, activation quantization remains to be challenging due to the activation outliers. Conventional remedies, e.g., mixing precisions for different channels, introduce extra overhead and reduce the speedup. In this work, we develop a simple yet effective strategy to facilitate per-tensor activation quantization by preventing the generation of problematic tokens. Precisely, we propose a method to find a set of key-value cache, coined CushionCache, which mitigates outliers in subsequent tokens when inserted as a prefix. CushionCache works in two steps: First, we greedily search for a prompt token sequence that minimizes the maximum activation values in subsequent tokens. Then, we further tune the token cache to regularize the activations of subsequent tokens to be more quantization-friendly. The proposed method successfully addresses activation outliers of LLMs, providing a substantial performance boost for per-tensor activation quantization methods. We thoroughly evaluate our method over a wide range of models and benchmarks and find that it significantly surpasses the established baseline of per-tensor W8A8 quantization and can be seamlessly integrated with the recent activation quantization method.

==> figures/per_step.tex <==
\begin{figure}[t]
\includegraphics[width=0.48\textwidth,height=5cm]{example-image-duck}  \caption{A placeholder. bar graph showing incremental quality gains per step.}
\end{figure}


==> figures/quantization_configs.tex <==
\begin{figure}[t]
\includegraphics[width=0.48\textwidth,height=5cm]{example-image-duck}  \caption{Explain the about the activation quantization configs.}
\end{figure}


==> sections/searchcost.tex <==
\section{Search cost of CushionCache}\label{app:searchcost}

\begin{table}[h]
\centering
\small
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Step 1} & \textbf{Step 2} & \textbf{Total Time} \\
\midrule
LLaMA2-7B & 2.68 hours & 3.34 hours & 6.02 hours \\
LLaMA3-8B & 12.09 hours & 3.70 hours & 15.79 hours \\
OPT-7B & 1.38 hours & 2.71 hours & 4.09 hours \\
\bottomrule
\end{tabular}
}
\caption{CushionCache Search Time}
\label{tab:search_cost}
\end{table}

We now bring our attention to the computational cost of searching for CushionCache. The algorithm consists of two components: (1) Greedy search of prompts, and (2) Quantization-aware prefix tuning.

In \cref{tab:search_cost}, we report the total wall-clock time for completing each step, measured on a server with four NVIDIA A6000 GPUs. From the table, we first observe that the greedy prefix search can be quite time-consuming, highly dependent on the side of the embedding table; LLaMA3-8B has a larger embedding table than others, and the time consumed for LLaMA3 is much larger than other two models. The second observation is that the quantization-aware prefix tuning step takes relatively small time for all models.

==> tables/LLaMA2-13B.tex <==
\begin{table*}[t]
    \small
    \centering
    \label{tab:llama3}
    \resizebox{0.99\textwidth}{!}{%

    \begin{tabular}{lccccccccc}
        \toprule
        \emph{LLaMA3-8B}     & {LAMBADA} & {HellaSwag} & {PIQA} & {WinoGrande} & {OpenBookQA} & {RTE}  & {COPA} & \textbf{Average$\uparrow$} & \textbf{WikiText$\downarrow$} \\
        \midrule
        FP16                & 74.7\%    & 59.3\%      & 79.7\% & 72.6\%       & 34.0\%       & 59.9\% & 88.0\% & 66.9\%                     & 10.99                         \\ \midrule
        W8A8                & 0.0\%     & 25.6\%      & 53.4\% & 50.3\%       & 14.0\%       & 49.5\% & 56.0\% & 35.5\%                     & 93080                         \\
        SmoothQuant           & 0.0\%{*}  & 26.0\%      & 51.7\% & 49.3\%       & 17.8\%       & 50.9\% & 55.0\% & 35.8\%                     & 84648                         \\
        \texttt{LLM.int8()}          & 74.7\%    & 59.2\%      & 79.7\% & 72.1\%       & 34.2\%       & 60.3\% & 87.0\% & 66.7\%                     & 11.10                         \\
        Outlier Suppression & 0.00\%    & 25.8\%      & 52.5\% & 48.6\%       & 16.6\%       & 53.4\% & 55.0\% & 36.0\%                     & 96151                         \\ \midrule
        Ours & 74.6\% & 58.9\% & 79.7\% & 71.2\% & 33.4\% & 59.9\% & 90.0\% & 66.8\% & 11.17 \\
        \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Per-tensor Activation Quantization.} We extensively benchmark the performance on 7 zero-shot benchmarks (by reporting the average accuracy) and 1 language modeling benchmark (perplexity).}
    
\end{table*}


==> tables/drq_srq.tex <==
\begin{table}[ht]
    \small
    \centering
    \label{tab:drq_srq}
    \resizebox{0.4\textwidth}{!}{%

    \begin{tabular}{lll}
    \toprule
    Per-tensor & Dynamic Range  & Static Range  \\ \midrule
    W8A8   & 8.01 & - \\
    Ours   & 5.68 & - \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{DRQ vs SRQ.}}
    
\end{table}

